Input Validation for Neural Networks via Runtime Local Robustness Verification

Local robustness verification can verify that a neural network is robust wrt. any perturbation to a specific input within a certain distance. We call this distance Robustness Radius. We observe that the robustness radii of correctly classified inputs are much larger than that of misclassified inputs which include adversarial examples, especially those from strong adversarial attacks. Another observation is that the robustness radii of correctly classified inputs often follow a normal distribution. Based on these two observations, we propose to validate inputs for neural networks via runtime local robustness verification. Experiments show that our approach can protect neural networks from adversarial examples and improve their accuracies.

==> fig/makefile <==
all: icml

SRC=	paper.bib \
	macros.tex \
	packages.tex

icml: paper.tex $(SRC)
	latex paper.tex && \
	bibtex --min-crossrefs=500 paper && \
	latex paper.tex && \
        latex paper.tex && \
	dvips -Ppdf -tletter -G0 paper.dvi -o paper.ps && \
	ps2pdf paper.ps paper.pdf

#------------------------------------------------------------------------
# Auxilliary targets
#------------------------------------------------------------------------
.PHONY: clean edit wc wca lab todo todos check
clean:
	rm -f *.ps *.dvi *.pdf *~ *.eps \#* *.swp *.log *.aux *.out && \
	rm -f *.blg *.toc *.bb *.lof
edit:
	emacs --background-color=Black --foreground-color=White makefile icml.tex macros.tex &
wedit:
	emacs --background-color=White --foreground-color=Black makefile icml.tex macros.tex &
wc:
	wc $(SRC) icml.tex
lab:
	grep label icml.tex > lab
todo:
	egrep "%%" icml.tex | wc
todos:
	grep "%" icml.tex > todos
check:
	grep "%" icml.tex | grep -v "%%"



==> packages.tex <==
% Encoding
% Layout, fonts, etc
\RequirePackage{amsfonts}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amstext}
%\RequirePackage{booktabs}
%\RequirePackage{calc}
%\RequirePackage{color}
%\RequirePackage{fancyhdr}
%\RequirePackage{float}
%\RequirePackage{hhline}
\RequirePackage{layouts}
\RequirePackage{listings}
%\RequirePackage{marvosym}
%\RequirePackage{mathrsfs}
\RequirePackage{mathtools}
%\RequirePackage{multicol}
\RequirePackage{microtype}
\RequirePackage{paralist}
\RequirePackage{pifont}
%\RequirePackage{proof}
\RequirePackage{pst-node}
%\RequirePackage{relsize}
\RequirePackage{stmaryrd}
\RequirePackage{subfigure}
%\RequirePackage{tabls}
%\RequirePackage{tabularx}
%\RequirePackage{tikz}
\RequirePackage{verbatim}
\RequirePackage{xspace}
\usepackage{etex}


